Revealing the Hidden Effects of Phishing Emails: An Analysis of Eye and Mouse Movements in Email Sorting Tasks

Users are the last line of defense as phishing emails pass filter mechanisms. At the same time, phishing emails are designed so that they are challenging to identify by users. To this end, attackers employ techniques, such as eliciting stress, targeting helpfulness, or exercising authority, due to which users often miss being manipulated out of malicious intent. This work builds on the assumption that manipulation techniques, even if going unnoticed by users, still lead to changes in their behavior. In this work, we present the outcomes of an online study in which we collected gaze and mouse movement data during an email sorting task. Our findings show that phishing emails lead to significant differences across behavioral features but depend on the nature of the email. We discuss how our findings can be leveraged to build security mechanisms protecting users and companies from phishing.

==> tables/classification.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{User Independent Classifiers comparison for behavioral features (mouse movement, gaze behavior, and both) between Decision Tree, Random Forest, SVM, and Gradient Boosting.}
\label{tab:classification}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccccc}
\hline
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}User-independent\\ Classifier\end{tabular}}}} & \multicolumn{2}{c}{\textbf{Decision Tree}} & \multicolumn{2}{c}{\textbf{Random Forest}} & \multicolumn{2}{c}{\textbf{SVM}} & \multicolumn{2}{c}{\textbf{Gradient Boosting}} \\
\multicolumn{1}{c}{} & Accuracy & AUC & Accuracy & AUC & Accuracy & AUC & Accuracy & AUC \\ \hline
\textbf{Gaze Features} & 60.94 ± 5.1 & 61.94 ± 3.8 & 63.75 ± 3.7 & \textbf{66.89 ± 5.8} & 49.45 ± 0.9 & 51.17 ± 0.9 & 64.85 ± 5.4 & 66.55 ± 3.9 \\
\textbf{Mouse Features} & 59.47 ± 4.3 & 59.47 ± 4.3 & 61.66 ± 6.8 & 65.44 ± 6.6 & 61.31 ±  8.4 & 64.81 ± 7.8 & 67.6 ± 6.6 & \textbf{68.02 ± 5.4} \\
\textbf{Both Features} & 57.54 ± 0.7 & 61.59 ± 1.7 & 61.65 ± 6.0 & 67.23 ± 6.9 & 47.95 ± 1.0 & 53.32 ± 2.3 & 65.25 ± 4.5 & \textbf{67.98 ± 5.3} \\ \hline
\end{tabular}%
}
\end{table}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{User dependent Classifiers comparison for behavioral features (mouse movement, gaze behavior, and both) between Decision Tree, Random Forest, Extra Trees, SVM, and Gradient Boosting.}
\label{tab:classification2}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lllllllll}
\hline
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}User-dependent\\ Classifier\end{tabular}}}} & \multicolumn{2}{c}{\textbf{Decision Tree}} & \multicolumn{2}{c}{\textbf{Random Forest}} & \multicolumn{2}{c}{\textbf{SVM}} & \multicolumn{2}{c}{\textbf{Gradient Boosting}} \\
\multicolumn{1}{c}{} & \multicolumn{1}{c}{Accuracy} & \multicolumn{1}{c}{AUC} & \multicolumn{1}{c}{Accuracy} & \multicolumn{1}{c}{AUC} & \multicolumn{1}{c}{Accuracy} & \multicolumn{1}{c}{AUC} & \multicolumn{1}{c}{Accuracy} & \multicolumn{1}{c}{AUC} \\ \hline
\textbf{Gaze Features} & 57.28 ± 18.67 & 57.28 ± 18.67 & 55.07 ± 20.87 & 53.93 ± 24.68 & 49.54 ± 16.77 & 51.01 ± 27.41 & 71.69 ± 16.79 & \textbf{65.89 ± 20.25} \\
\textbf{Mouse Features} & 57.02 ± 19.18 & 57.02 ± 19.18 & 61.32 ± 16.60 & 62.92 ± 27.79 & 53.68 ± 18.82 & 46.97 ± 28.00 & 70.86 ± 16.93 & \textbf{68.29 ± 21.78} \\
\textbf{Both Features} & 53.68 ± 19.70 & 53.68 ± 19.70 & 62.17 ± 17.19 & 58.60 ± 27.89 & 49.98 ± 16.45 & 51.71 ± 28.40 & 70.53 ± 16.27 & \textbf{65.54 ± 22.34} \\ \hline
\end{tabular}%
}
\end{table}

==> tables/gazeFeatures.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[]
\caption{Wilcoxon Signed-rank Test for The Gaze Features across our 3 models (Significant results in bold).}
\label{tab:GazeFeatures}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccccccc}
\toprule
\multirow{2}{*}{\textbf{Gaze Features}} & \multicolumn{3}{c}{\textbf{Labeling Task}} & \multicolumn{3}{c}{\textbf{Perceived Ground Truth}} & \multicolumn{3}{c}{\textbf{Ground Truth}} \\
 & \textbf{\begin{tabular}[c]{@{}c@{}}Mean\\ Spam\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Mean\\ Not Spam\end{tabular}} & \textbf{Wilcoxon} & \textbf{\begin{tabular}[c]{@{}c@{}}Mean\\ Spam\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Mean\\ Not Spam\end{tabular}} & \textbf{Wilcoxon} & \textbf{\begin{tabular}[c]{@{}c@{}}Mean\\ Spam\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Mean\\ Not Spam\end{tabular}} & \textbf{Wilcoxon} \\ 
 \midrule
\textbf{Fixation Duration} & 42233.4 & 39691.4 & P \textgreater 0.05, Z = -.404 & 47334.7 & 28043.9 & P \textgreater 0.05, Z = -1.662 & \textbf{41954.4} & \textbf{35207.7} & \textbf{P \textless 0.05, Z = -2.108} \\
\textbf{Avg Fixation Duration} & 5496.4 & 8107.3 & P \textgreater 0.05, Z = -.374 & \textbf{8827.3} & \textbf{4602.9} & \textbf{P \textless 0.05, Z = -2.889} & 6925.5 & 5245.3 & P \textgreater 0.05, Z = -1.954 \\
\textbf{Saccade Duration} & 24318.4 & 25811.8 & P \textgreater 0.05, Z = -.1.679 & 22106.4 & 31646.6 & P \textgreater 0.05, Z = -1.206 & 20725.5 & 30715.6 & P \textgreater 0.05, Z = -.156 \\
\textbf{Avg Saccade Duration} & 1925.1 & 1953.6 & P \textgreater 0.05, Z = -1.945 & 1771.5 & 2580.2 & P \textgreater 0.05, Z = -.057 & 1581.8 & 2408.5 & P \textgreater 0.05, Z = -.370 \\
\textbf{Fixation Count} & \textbf{146.6} & \textbf{167.2} & \textbf{P \textless 0.01, Z = -3.210} & 156.5 & 164.1 & P \textgreater 0.05, Z = -1.524 & 167.4 & 162.94 & P \textgreater 0.05, Z = -212 \\
\textbf{Avg Fixation Count} & 162.4 & 162.4 & P \textgreater 0.05, Z = -.1.174 & 158 & 172.9 & P \textgreater 0.05, Z = -1.314 & 171.9 & 162.4 & P \textgreater 0.05, Z = -610 \\
\textbf{Saccade Length} & .5305 & .5079 & P \textgreater 0.05, Z = -.583 & \textbf{.4854} & \textbf{.4668} & \textbf{P \textless 0.05, Z = -3.021} & .4776 & .4890 & P \textgreater 0.05, Z = -.932 \\
\textbf{Avg Saccade Length} & .4695 & .4921 & P \textgreater 0.05, Z = -.1.174 & .5146 & .5332 & P \textgreater 0.05, Z = -1.314 & .5224 & .5110 & P \textgreater 0.05, Z = -.610 \\ 
\bottomrule
\end{tabular}%
}
\end{table*}

==> tables/gazeFeaturesCategories.tex <==
% 
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{gr% Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% % \usepackage{graphicx}
% \begin{table}[]
% \centering
% \caption{Wilcoxon test results for eye gaze movement analysis over the different email categories (Significant results in bold).}
% \label{tab:GazeFeatures}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{lllll}
% \hline
% \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Gaze Features}}} & \multicolumn{4}{c}{\textbf{Wilcoxon}} \\
% \multicolumn{1}{c}{} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Overall\\ Phishing/non phishing\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Imp\\ Phishing/non phihsing\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Ads\\ Phishing/non phishing\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Neutral\\ Phishing/non phishing\end{tabular}}} \\ \hline
% \textbf{Fixation Duration} & Z=-.544, P=.586 & Z=-1.320, P=.187 & Z=-1.196, P=.232 & Z=-1.094, P=.274 \\
% \textbf{Avg Fixation Duration} & \textbf{Z=-2.372, P=.018} & Z=-1.697, P=.090 & Z=-1.080, P=.280 & Z=-1.109, P=.267 \\
% \textbf{Saccade Duration} & Z=-1.884, P=.060 & Z=-.626, P=.531 & Z=-.457, P=.648 & \textbf{Z=-2.406, P=.016} \\
% \textbf{Avg Saccade Duration} & \textbf{Z=-2.330, P=.020} & Z=-1.124, P=.261 & \textbf{Z=-3.227, P=.001} & \textbf{Z=-2.814, P=.005} \\
% \textbf{Fixation Count} & \textbf{Z=-4.347, P=<.001} & Z=-1.848, P=.065 & \textbf{Z=-4.372, P=<.001} & Z=-.596, P=.551 \\
% \textbf{Avg Fixation Count} & Z=-.251, P=.802 & Z=-.008, P=.994 & Z=-.138, P=.890 & Z=-.581, P=.561 \\
% \textbf{Saccade Length} & \textbf{Z=-4.186, P=<.001} & Z=-1.712, P=.087 & \textbf{Z=-4.430, P=<.001} & Z=-.536, P=.592 \\
% \textbf{Avg Saccade Length} & Z=.251, P=.802 & Z=-.008, P=.994 & Z=-.138, P=.890 & Z=-.581, P=.561 \\ \hline
% \end{tabular}%
% }
% \end{table}




% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\label{tab:GazeFeatures1}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lllllll}
\hline
\multirow{3}{*}{\textbf{Gaze Features}} & \multicolumn{6}{c}{\textbf{Wilcoxon}} \\
 & \multicolumn{3}{c}{\textbf{Overall Phishing/non phishing}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Imp\\ Phishing/\\ non-phishing\end{tabular}}}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Ads\\ Phishing/\\ non-phishing\end{tabular}}}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Neutral\\ Phishing/\\ non-phishing\end{tabular}}}} \\
 & \textit{\textbf{\begin{tabular}[c]{@{}l@{}}Mean non\\ Phishing\end{tabular}}} & \textit{\textbf{\begin{tabular}[c]{@{}l@{}}Mean\\ Phishing\end{tabular}}} & \textit{\textbf{Wilcoxon}} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} \\ \hline
\textbf{Fixation Duration} & 52608.12 & 57109.3 & Z=-.54, P=.58 & Z=-1.32, P=.18 & Z=-1.19, P=.23 & Z=-1.09, P=.27 \\
\textbf{Avg Fixation Duration} & \textbf{10595.06} & \textbf{8610.93} & \textbf{Z=-2.37, P=.018} & Z=-1.69, P=.09 & Z=-1.08, P=.28 & Z=-1.10, P=.26 \\
\textbf{Saccade Duration} & 30881.52 & 20409.46 & Z=-1.88, P=.06 & Z=-.62, P=.53 & Z=-.45, P=.64 & \textbf{Z=-2.40, P=.016} \\
\textbf{Avg Saccade Duration} & \textbf{7715.25} & \textbf{2753.63} & \textbf{Z=-2.33, P=.02} & Z=-1.12, P=.26 & \textbf{Z=-3.22, P=.001} & \textbf{Z=-2.81, P=.005} \\
\textbf{Fixation Count} & \textbf{134.58} & \textbf{189.12} & \textbf{Z=-4.34, P\textless{}.001} & Z=-1.84, P=.06 & \textbf{Z=-4.372 P\textless{}.001} & Z=-.59, P=.55 \\
\textbf{Avg Fixation Count} & .49 & .49 & Z=-.25, P=.80 & Z=-.00, P=.99 & Z=-.13, P=.89 & Z=-.58, P=.56 \\
\textbf{Saccade Length} & \textbf{119.2} & \textbf{157.2} & \textbf{Z=-4.18, P\textless{}.001} & Z=-1.71, P=.08 & \textbf{Z=-4.43, P\textless{}.001} & Z=-.53, P=.59 \\
\textbf{Avg Saccade Length} & .51 & .51 & Z=.25, P=.80 & Z=-.00, P=.99 & Z=-.13, P=.89 & Z=-.58, P=.56 \\ \hline
\end{tabular}
}
\end{table*}


% % Please add the following required packages to your document preamble:
% % \usepackage{graphicx}
% \begin{table}[]
% \centering
% \caption{Friedman test results for eye gaze movement analysis with Wilcoxen Sign-rank tests for pairwise comparisons (Significant results in bold).}
% \label{tab:GazeFeatures}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{lccllccl}
% \hline
% \multicolumn{1}{c}{\textbf{Gaze Features}} & \textbf{Friedman (��2(2); P)} & \textbf{Neutral/Ads} & \textbf{Imp/Ads} & \textbf{Imp/Neutral} & \textbf{Phishing/Imp} & \textbf{Phishing/Neutral} & \textbf{Phishing/Ads} \\ \hline
% \textbf{Fixation Duration} & ��2(2)=4.3, P>.05 & Z=-.094, P=.925 & Z=-.152, P=.879 & Z=-.065, P=.948 & Z=-.761, P=.446 & Z=-.558, P=.577 & Z=-.877, P=.380 \\
% \textbf{Avg Fixation Duration} & ��2(2)=.6, P>.05 & Z=-.341, P=.733 & Z=-.268, P=.788 & Z=-.834, P=.404 & Z=-1.399, P=.162 & Z=-.109, P=.913 & Z=-.377, P=.706 \\
% \textbf{Saccade Duration} & \textbf{��2(2)=9.8, P=.02} & \textbf{Z=-1.980, P=.048} & Z=-.413, P=.679 & \textbf{Z=-2.458, P=.014} & Z=-.718, P=.473 & Z=-1.870, P=.061 & Z=-.210, P=.833 \\
% \textbf{Avg Saccade Duration} & ��2(2)=5.8, P>.05 & Z=-1.806, P=.071 & Z=-1.167, P=.243 & Z=-1.298, P=.194 & Z=-.805, P=.421 & \textbf{Z=-2.037, P=.042} & Z=-.167, P=.868 \\
% \textbf{Fixation Count} & \textbf{��2(2)=31.1, P<.01} & Z=-.616, P-.538 & \textbf{Z=-3.256, P=.001} & \textbf{Z=-4.575, P<.001} & \textbf{Z=-4.691, P<,001} & Z=-1.682, P=.093 & Z=-1.109, P=.267 \\
% \textbf{Avg Fixation Count} & ��2(2)=3.3, P>.05 & Z=-1.138, P=.255 & Z=-1.428,P=.153 & Z=-1.283, P=.199 & Z=-1.051, P=.293 & Z=-.377, P=.706 & Z=-.921, P=.357 \\
% \textbf{Saccade Length} & \textbf{��2(2)=30.7, P<.01} & Z=1.632, P=.103 & \textbf{Z=-2.690, P=.007} & \textbf{Z=-4.459, P=<.001} & \multicolumn{1}{l}{\textbf{Z=-4.76, P=<.001}} & Z=-1.298, P=.194 & Z=-1.864,  P=.062 \\
% \textbf{Avg Saccade Length} & ��2(2)=3.4, P>.05 & Z=-1.138, P=.255 & Z=-1.428, P=.153 & Z=-1.283, P=.199 & Z=-1.051, P=.293 & Z=-.377, P=.706 & Z=-.921, P=.357 \\ \hline
% \end{tabular}%
% }
% \end{table}

==> tables/task1labelling.tex <==
\begin{table}[ht]
    \small
    \begin{minipage}[t]{.48\linewidth}
    \caption{Emails classification based on the target inbox chosen by participants in Group 1.}
    \label{tab:group1-labelled}
    \begin{tabular}{lrrrr}
    \toprule
    \textbf{\begin{tabular}[c]{@{}l@{}}Email Type/\\ Labelled As\end{tabular}} & \multicolumn{1}{l}{\textbf{Phishing}} & \multicolumn{1}{l}{\textbf{Important}} & \multicolumn{1}{l}{\textbf{Neutral}} & \multicolumn{1}{l}{\textbf{Ads}} \\ 
    \midrule
    \textbf{Bin} & 15.9\% & 1.7\% & 6\% & 93.4\% \\
    \textbf{Important} & 55.3\% & 77.5\% & 31.9\% & 0.3\% \\
    \textbf{Neutral} & 28.8\% & 20.8\% & 21.1\% & 6.3\% \\ 
    \bottomrule
    \end{tabular}
\end{minipage}
\hspace{0.2cm}
\begin{minipage}[t]{.48\linewidth}
    \caption{Emails classification based on the target inbox chosen by participants in Group 2}
    \label{tab:group2-labelled}
    \begin{tabular}{lrrrr}
    \toprule
    \textbf{\begin{tabular}[c]{@{}l@{}}Email Type/\\ Labelled As\end{tabular}} & \multicolumn{1}{l}{\textbf{Phishing}} & \multicolumn{1}{l}{\textbf{Important}} & \multicolumn{1}{l}{\textbf{Neutral}} & \multicolumn{1}{l}{\textbf{Ads}} \\ 
    \midrule
    \textbf{Bin} & 6\% & 12.5\% & 6.6\% & 38.2\% \\
    \textbf{Important} & 49\% & 67.8\% & 25.6\% & 7.7\% \\
    \textbf{Neutral} & 36.8\% & 19.4\% & 66.1\% & 0.3\% \\
    \textbf{Spam} & 8.2\% & 0.3\% & 1.7\% & 53.8\% \\ 
    \bottomrule
    \end{tabular}
\end{minipage}
\end{table}




==> tables/task2labelling.tex <==
\begin{table}[ht]
\small
\begin{minipage}[t]{.48\linewidth}
    \caption{Results for Task 2 of Group 1. Participants had to classify emails as \textit{Spam} and \textit{Not Spam}.}
    \label{tab:group1-task2}
    \begin{tabular}{lrrrr}
    \toprule
    \textbf{\begin{tabular}[c]{@{}l@{}}Email Type/\\ Labelled As\end{tabular}} & \multicolumn{1}{l}{\textbf{Phishing}}  & \multicolumn{1}{l}{\textbf{Important}} & \multicolumn{1}{l}{\textbf{Neutral}} & \multicolumn{1}{l}{\textbf{Ads}} \\ 
    \midrule
    \textbf{Spam} & 20.2\% & 1.1\% & 5.1\% & 87.2\% \\
    \textbf{Not Spam} & 79.8\% & 98.9\% & 94.9\% & 12.8\% \\ 
    \bottomrule
    \end{tabular}
\end{minipage}
\hspace{0.2cm}
\begin{minipage}[t]{.48\linewidth}
    \caption{Results for Task 2 of Group 2. Participants had to classify emails as \textit{Spam} and \textit{Not Spam}.}
    \label{tab:group2-task2}
    \begin{tabular}{lrrrr}
    \toprule
    \textbf{\begin{tabular}[c]{@{}l@{}}Email Type/\\ Labelled As\end{tabular}} & \multicolumn{1}{l}{\textbf{Phishing}} & \multicolumn{1}{l}{\textbf{Important}} & \multicolumn{1}{l}{\textbf{Neutral}} & \multicolumn{1}{l}{\textbf{Ads}} \\ 
    \midrule
    \textbf{Spam} & 2.7\% & 0.3\% & 2.6\% & 88.7\% \\
    \textbf{Not Spam} & 97.3\% & 99.7\% & 97.4\% & 11.3\% \\ 
    \bottomrule
    \end{tabular}
\end{minipage}
\end{table}

\begin{table}[htb]
    \caption{Results for Task 2 of Group 3. Participants had to classify emails as \textit{Spam} and \textit{Not Spam}.}
    \label{tab:group3}
    \small
    \begin{tabular}{lrrrr}
    \toprule
    \textbf{\begin{tabular}[c]{@{}l@{}}Email Type/\\ labeled As\end{tabular}} & \multicolumn{1}{l}{\textbf{Phishing}} & \multicolumn{1}{l}{\textbf{Important}} & \multicolumn{1}{l}{\textbf{Neutral}} & \multicolumn{1}{l}{\textbf{Ads}} \\ 
    \midrule
    \textbf{Spam} & 34.9\% & 1.6\% & 8.5\% &  87.1\% \\
    \textbf{Not Spam} & 65.1\% & 98.4\% & 91.5\% &12.9\% \\ 
    \bottomrule
    \end{tabular}
\end{table}

